On Fast Convergence of Proximal Algorithms for SQRT-Lasso Optimization: Don't Worry About Its Nonsmooth Loss Function

Many machine learning techniques sacrifice convenient computational structures to gain estimation robustness and modeling flexibility. However, by exploring the modeling structures, we find these "sacrifices" do not always require more computational efforts. To shed light on such a "free-lunch" phenomenon, we study the square-root-Lasso (SQRT-Lasso) type regression problem. Specifically, we show that the nonsmooth loss functions of SQRT-Lasso type regression ease tuning effort and gain adaptivity to inhomogeneous noise, but is not necessarily more challenging than Lasso in computation. We can directly apply proximal algorithms (e.g. proximal gradient descent, proximal Newton, and proximal Quasi-Newton algorithms) without worrying the nonsmoothness of the loss function. Theoretically, we prove that the proximal algorithms combined with the pathwise optimization scheme enjoy fast convergence guarantees with high probability. Numerical results are provided to support our theory.

==> experiment.tex <==
%!TEX root = ./sqrtlasso_paper.tex
%\vspace{-0.15in}
\section{Numerical Experiments}
%\vspace{-0.1in}

We investigate the computational performance of the proposed PISTA algorithm through numerical experiments over both simulated and real data example. All simulations are implemented in \texttt{C} with double precision using a PC with an Intel 3.3GHz Core i5 CPU and 16GB memory.

For simulated data, we generate a training dataset of $200$ samples, where each row of the design matrix $\Xb_{i,\star}$, $i = 1,\ldots,200$, independently from a $2000$-dimensional normal distribution $N(\zero,\bSigma)$ where $\bSigma_{jj} = 1$ and $\bSigma_{jk} = 0.5$ for all $k\neq j$. We set $s^*=3$ with $\theta_1^*=3$, $\theta_2^*=-2$, and $\theta_4^*=1.5$, and $\theta_j^*=0$ for all $j\neq 1,2,4$. A validation set of $200$ samples for the regularization parameter selection and a testing set of $10,000$ samples are also generated to evaluate the prediction accuracy. 

We set $\sigma=0.5, 1, 2, 4$ respectively to illustrate the tuning insensitivity. The regularization parameter of both Lasso and SQRT-Lasso is chosen over a geometrically decreasing sequence $\{\lambda\}_{t=0}^{50}$with $\lambda_{50} = \sigma\sqrt{\log d/n}/2$ for Lasso and $\lambda_{50}=\sqrt{\log d/n}/2$ for SQRT-Lasso. The optimal regularization parameter is determined by ${\lambda}_{\opt}=\lambda_{\hat{N}}$ as $\hat{N} = \argmin_{K\in\{0,\ldots,50\}}\norm{\tilde{\by}-\tilde{\Xb}\hat{\btheta}}_2^2$, where $\hat{\btheta}$ denotes the obtained estimate using the regularization parameter $\lambda$, and $\tilde{\by}$ and $\tilde{\Xb}$ denote the response vector and design matrix of the validation set. For both Lasso and SQRT-Lasso, we set the stopping precision $\varepsilon = 10^{-5}$ for all $K = 1,\ldots,30$ and $\varepsilon = 10^{-5}$ for all $K = 31,\ldots,50$.

First of all, we compare PISTA with ADMM proposed in \cite{li2015flare}\footnote{We do not have any results for the algorithm proposed in \cite{belloni2011square}, because it failed to finish 500 simulations in 12 hours. The implementation was based on SDPT3.}. We conduct 500 simulations for all $\sigma$'s. The results are presented in Table~\ref{table:sqrt_lasso_cmp}. The PISTA and ADMM algorithms attain similar objective values, but PISTA is about 20 times faster than ADMM. Both algorithms also achieve similar estimation errors. Throughout all 500 simulations, we have $\norm{\by-\Xb\hat{\btheta}_{[\hat{N}]}}_2 \gg 0$. This implies that all obtained optimal estimators are far from the nonsmooth point of the optimization problem.

%\vspace{-0.15in}
\begin{table*}[!htb]
	\caption{Quantitative comparison between Lasso (PISTA-L) and SQRT-Lasso (PISTA-S and ADMM) over 500 simulations. The estimation error is defined as $\norm{\hat{\btheta} - \btheta^*}_2$. The prediction error is defined as $\norm{\tilde{\by} - \tilde{\Xb} \hat{\btheta}_{[\hat{N}]}}_2/\sqrt{n}$. The residual is defined as $\norm{\by-\Xb\hat{\btheta}_{[\hat{N}]}}_2$ for PISTA-S only. PISTA-S attains nearly the same estimation and prediction errors as ADMM, but is significantly faster than ADMM over all different settings. Besides, we also find that all obtained estimators are outside the smoothed region throughout all 500 simulations.}
%	\vspace{-0.03in}
	\begin{center}
		\renewcommand{\arraystretch}{1.2}
		{
			\begin{tabular}{c|c|c|c|c|c|c|c|c}
				\Xhline{1 pt}
				Variance & \multicolumn{2}{c|}{Est. Err.} & \multicolumn{2}{c|}{Pred. Err.} & \multicolumn{3}{c|}{Time (Second)} & Residual \\
				\cline{2-9}
				of Noise & PISTA-L & PISTA-S & PISTA-L & PISTA-S & PISTA-L & PISTA-S & ADMM & PISTA-S \\
				\Xhline{1 pt}
				\multirow{2}{*}{$\sigma=0.5$} & 0.2761 & 0.2760 & 0.5403 & 0.5399 & 0.8817 & 0.9526 & 17.260 & 5.2505 \\
				& (0.0651) & (0.0537) & (0.0172) & (0.0143) & (0.2824) & (0.2646) & (3.1723) & (0.9591) \\
				\hline
				\multirow{2}{*}{$\sigma=1$\hspace{0.1in}} & 0.5271 & 0.5319 & 1.0722 & 1.0757 & 0.9146 & 1.0170 & 19.762 & 10.5209 \\
				& (0.1174) & (0.1065) & (0.0303) & (0.0280) & (0.3185) & (0.2959) & (4.4387) & (1.7760) \\
				\hline
				\multirow{2}{*}{$\sigma=2$\hspace{0.1in}} & 1.0962 & 1.1065 & 2.1551 & 2.1492 & 1.1772 & 1.1263 & 24.406 & 20.886 \\
				& (0.2252) & (0.2141) & (0.0595) & (0.0589) & (0.4582) & (0.4128) & (4.2786) & (3.6506)  \\
				\hline
				\multirow{2}{*}{$\sigma=4$\hspace{0.1in}} & 2.1275 & 2.1356 & 4.2928 & 4.2963 & 1.2913 & 1.2544 & 26.101 & 45.7623 \\
				& (0.4247) & (0.4033) & (0.1112) & (0.1079) & (0.4855) & (0.5074) & (5.7725) & (5.6333) \\
				\Xhline{1 pt}
		\end{tabular}}\label{table:sqrt_lasso_cmp}
	\end{center}
	
	\vspace{-0.015in}
	
	\caption{Timing comparison between PISTA-S and ADMM on biology data under different levels of sparsity recovery. PISTA-S is significantly faster than ADMM over all different settings and data sets.}
%	\vspace{-0.03in}
	\begin{center}
		\renewcommand{\arraystretch}{1.18}
		{
			\begin{tabular}{c|c|c|c|c|c|c|c|c}
				\Xhline{1 pt}
				\multirow{2}{*}{} & \multicolumn{2}{c|}{Estrogen} & \multicolumn{2}{c|}{Arabidopsis} & \multicolumn{2}{c|}{Leukemia} & \multicolumn{2}{c}{Hereditary} \\
				\cline{2-9}
				& PISTA-S & ADMM & PISTA-S & ADMM & PISTA-S & ADMM & PISTA-S & ADMM \\
				\Xhline{1 pt}
				%\multirow{2}{*}{Time}
				{\rm Sparsity}~~1\% & 16.562 & 175.98 & 18.404 & 373.83 & 30.609 & 431.45 & 43.161 & 498.32 \\
				{\rm Sparsity}~~3\% & 70.622 & 338.96 & 81.557 & 707.52 & 86.406 & 812.69 & 141.65 & 895.09 \\
				{\rm Sparsity}~10\% & 188.03 & 703.24 & 226.97 & 1378.1 & 257.23 & 1653.1 & 413.85 & 1921.6 \\
				\Xhline{1 pt}
		\end{tabular}}\label{table:pissta_admm}
	\end{center}%\vspace{-0.1in}
\end{table*}

Next, we compare the computational and statistical performance between Lasso and SQRT-Lasso (both solved by PISTA). The results averaged over 500 simulations are summarized in Tables~\ref{table:sqrt_lasso_cmp}. In terms of statistical performance, Lasso and SQRT-Lasso attains similar estimation and prediction error. In terms of computational performance, the PISTA algorithm for solving SQRT-Lasso is as efficient as Lasso, which matches our computational analysis. 

Moreover, we also examine the optimal regularization parameters for Lasso and SQRT-Lasso. We visualize the distribution of all 500 selected ${\lambda}_{\opt}$'s using the kernel density estimator. Particularly, we adopt the Gaussian kernel, and the kernel bandwidth is selected based on the 10-fold cross validation. Figure~\ref{fig:dist_lamb} illustrates the estimated density functions. The horizontal axis corresponds to the rescaled regularization parameter $\frac{{\lambda}_{\opt}}{\sqrt{\log d/n}}$. We see that the optimal regularization parameters of Lasso significantly vary with different $\sigma$. In contrast, the optimal regularization parameters of SQRT-Lasso are more concentrated. This is consistent with the claimed tuning insensitivity. 

Finally, we compare PISTA with ADMM over real data sets for precision matrix estimation. Particularly,  we use four real world biology data sets preprocessed by \cite{li2010inexact}: Estrogen ($d = 692$), Arabidopsis ($d=834$), Leukemia ($d = 1,225$), Hereditary ($d = 1,869$). We set three different values for $\lambda_N$ such that the obtained estimators achieve different levels of sparse recovery. We set $N=50$, and $\varepsilon = 10^{-4}$ for all $K$'s. The timing performance is summarized in Table~\ref{table:pissta_admm}. As can be seen, PISTA is 5 to 20 times faster than ADMM on all four data sets\footnote{We do not have any results for the algorithm proposed in \cite{belloni2011square}, because it failed to finish the experiments on all four data sets in 12 hours. The implementation was also based on SDPT3.}.

\begin{figure}[H]
	\centering
	\subfigure[Lasso: Distribution of $\frac{{\lambda}_{\opt}}{\sqrt{\log d/n}}$]{
		\includegraphics[width=0.8\linewidth]{Figs/{lasso_lamb4}.pdf}
	} \\
	\subfigure[SQRT-Lasso: Distribution of $\frac{{\lambda}_{\opt}}{\sqrt{\log d/n}}$]{
		\includegraphics[width=0.8\linewidth]{Figs/{sqrt_lamb4}.pdf}
	}
	\vspace{-0.08in}
	\caption{Estimated distributions of $\frac{{\lambda}_{\opt}}{\sqrt{\log d/n}}$ over different values of $\sigma$ for Lasso and PISTA.}\label{fig:dist_lamb} \vspace{-0.05in}
\end{figure}
